FFB6D: A Full Flow Bidirectional Fusion Network for 6D Pose Estimation

In this work, we present FFB6D, a Full Flow Bidirectional fusion network designed for 6D pose estimation from a single RGBD image. Our key insight is that appearance information in the RGB image and geometry information from the depth image are two complementary data sources, and it still remains unknown how to fully leverage them. Towards this end, we propose FFB6D, which learns to combine appearance and geometry information for representation learning as well as output representation selection. Specifically, at the representation learning stage, we build bidirectional fusion modules in the full flow of the two networks, where fusion is applied to each encoding and decoding layer. In this way, the two networks can leverage local and global complementary information from the other one to obtain better representations. Moreover, at the output representation stage, we designed a simple but effective 3D keypoints selection algorithm considering the texture and geometry information of objects, which simplifies keypoint localization for precise pose estimation. Experimental results show that our method outperforms the state-of-the-art by large margins on several benchmarks. Code and video are available at \url{https://github.com/ethnhe/FFB6D.git}.

==> tmp_table_fig.tex <==

\newcommand{\cmpMDL}{1}
\begin{figure}
    \centering
    \subfigure[The DenseFusion \cite{wang2019densefusion} Network]{
        \begin{minipage}[]{\cmpMDL\linewidth}
            \centering
            \label{fig:dense_fusion}
            \includegraphics[scale=.75]{images/DensFusion.png}\\
        \end{minipage}%
    }%
    
    \subfigure[The Proposed Full Flow Bidirectional Fusion Network]{
        \begin{minipage}[]{\cmpMDL\linewidth}
            \centering
            \label{fig:FFF6Dsimp}
            \includegraphics[scale=.75]{images/FFB6D_cmp.png}\\
        \end{minipage}%
    }%
    \caption{
        \textbf{Network comparison} (a) The pipeline of DenseFusion \cite{wang2019densefusion}. The two networks extract features from different modalities of data separately without any communication, util the final layers of the encoding-decoding architecture. (b) The pipeline of the proposed FFB6D. Bidirectional fusion modules are added as bridges for information communication in the full flow of the two networks. Supplementary information from each other is shared between the two networks for better appearance and geometry representation learning, which is crucial for 6D pose estimation.
    }
    \label{fig:network_cmp}
\end{figure}


\begin{comment}
\begin{figure*}[htbp]
    \centering %居中
    
    \subfigure[Effect of RGB to point cloud feature fusion.]{ %第二张子图
    %\begin{subfigure}
        \begin{minipage}[b]{.35\textwidth}
            \centering %子图居中
            \includegraphics[scale=0.55]{images/r2p_res.png} %以pic.jpg的0.5倍大小输出
            %\caption{Effect of RGB to point cloud feature fusion.}
            \label{fig:effp2r}
        \end{minipage}
    }
    %\end{subfigure}
    \quad
    \subfigure[Effect of point cloud to RGB feature fusion.]{ %第一张子图
    %\begin{subfigure}
        \begin{minipage}[b]{.63\textwidth}
            \centering %子图居中
            \includegraphics[scale=0.55]{images/p2r_res.png} %以pic.jpg的0.5倍大小输出
            %\caption{Effect of point cloud to RGB feature fusion.}
            \label{fig:effr2p}
        \end{minipage}
    }
    %\end{subfigure}
    %}
    
    \caption{Qualitative results of full flow bidirectional fusion. (a) RGB completes the missing part of depth due to reflective surface and improve the pose accuracy. (b) Geometry information in depth helps distinguish similar appearance objects, release the capability of CNN to more significant feature for pose.} % %大图名称
    \label{fig:effbidirectional} %图片引用标记
\end{figure*}
\end{comment}





\begin{figure}
    \centering
    \includegraphics[scale=0.72]{images/network_cmp.png}
    \caption{
        \textbf{Network comparison} (a) The pipeline of DenseFusion \cite{wang2019densefusion}. The two networks extract features from different modalities of data separately without any communication, util the final layers of the encoding-decoding architecture. (b) The pipeline of the proposed FFB6D. Bidirectional fusion modules are added as bridges for information communication in the full flow of the two networks. Supplementary information from each other is shared between the two networks for better appearance and geometry representation learning, which is crucial for 6D pose estimation.
    }
    \label{fig:network_cmp}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mnps}{1}
\begin{figure*}
    \centering
    \subfigure[]{
        \begin{minipage}[]{\mnps\linewidth}
            \centering
            \label{fig:network_full}
            \includegraphics[scale=.55]{images/FFB6D_network_full.png}\\
        \end{minipage}%
    }%
    
    \subfigure[]{
        \begin{minipage}[]{\mnps\linewidth}
            \centering
            \label{fig:network_fusion}
            \includegraphics[scale=.65]{images/FFB6D_network_fusion.png}\\
        \end{minipage}%
    }%
    \caption{\textbf{Overview of FFB6D.}}
    \label{fig:network}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\mnps}{1}
\begin{figure*}
    \centering
    \begin{subfigure}[Overview of FFB6D]{}
        \begin{minipage}{1.0\linewidth}
            \centering
            \includegraphics[scale=.55]{images/FFB6D_network_full.png}
            \label{fig:network_full}
        \end{minipage}
    \end{subfigure}
    
    \bigskip
    
    \begin{subfigure}[Bidir]
        \begin{minipage}{1.0\linewidth}
        \centering
        \includegraphics[scale=.65]{images/FFB6D_network_fusion.png}
        \label{fig:network_full}
        \end{minipage}
    \end{subfigure}
 
        \   
    \caption{\textbf{Overview of FFB6D.}}
    \label{fig:network}
\end{figure*}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\newcommand{\fdeaC}{1.15}
\begin{table}[tp]
  \centering
  \fontsize{6.9}{6.8}\selectfont
  \begin{tabular}{C{\fdeC cm}|C{\fdeC cm}|C{\fdeC cm}|C{\fdeC cm}|C{\fdeC cm} }
    \hline
    \multicolumn{3}{c|}{Fusion Stage} & \multicolumn{2}{c}{Pose Result} \cr\hline
    FE       & FD        & DF      & ADD-S    & ADD(S) \cr\hline
    \texttimes & \texttimes  & \texttimes  & 91.9     & 87.5 \\
    \checkmark & \texttimes  & \texttimes  & 96.2     & 92.2 \\
    \texttimes & \checkmark  & \texttimes  & 93.0     & 89.2 \\
    \texttimes & \texttimes  & \checkmark  & 94.0     & 90.8 \\
    \checkmark & \checkmark  & \texttimes  & \textbf{96.6} & \textbf{92.7} \\
    \checkmark & \checkmark  & \checkmark  & 94.3     & 91.1  
    \cr\hline 
  \end{tabular}
  \caption{Effect of fusion on different level on the YCB-Video dataset. FE means fusion during encoding, FD means fusion during decoding, and DF means Dense Fusion on the two final feature maps.}
  \label{tab:EffFuseEcDc}
\end{table}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\begin{comment}
\subsection{3D Bounding Box Detection}
Recent studies in 3D object detection also detect the 8 corners of 3D bounding boxes of objects \cite{song2014sliding,song2016deep,zhou2018voxelnet,qi2018frustum}. However, the estimated 3D bounding boxes are
viewpoint-dependent and do not encode the precise orientation of objects. Most related to our methods, VoteNet \cite{qi2019deep} also proposes a deep hough voting network for 3D object detection. However, it didn't utilize the rich RGB information. It first votes for the center of objects and learned the feature of such virtual points. These virtual center further vote for the 8 corners of the bounding box. However, features of virtual center points are hard to learn and they are even farther to the corners of the bounding box, compared with points on the object. As a result, point-based networks difficult to aggregate scene context in the vicinity of these virtual corner points. Instead, we vote for 3D keypoints selected from vertexes on the object using visible points on it, which is easier for neural network to learn.
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%\newcommand{\mnps}{0.19}
\newcommand{\mnps}{0.17}
%\newcommand{\gw}{1.27}
\newcommand{\gw}{1.17}
\begin{figure*}[htbp]
\centering
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_361.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_361.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_361.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_650.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_650.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_650.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_948.png}\\
        \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_948.png}\\
        \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_948.png}\\
        \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
    }%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_1323.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_1323.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_1323.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\subfigure[]{
    \begin{minipage}[]{\mnps\linewidth}
        \centering
        \includegraphics[width=\gw in]{images/df_2342.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/ours_2342.png}\\
        % \vspace{0.02cm}
        \includegraphics[width=\gw in]{images/gt_2342.png}\\
        % \vspace{0.02cm}
        %\caption{fig1}
    \end{minipage}%
}%
\centering
\caption{
    \textbf{Qualitative results on the YCB-Video Dataset.} Points on different meshes are in different colors. They are projected back to the image after being transformed by the predicted pose. Images on the top row are results of DenseFusion (iterative) \cite{wang2019densefusion}. The middle row shows the results of our model without any iterative refinement procedure. The ground truths are shown in the bottom row. Our model distinguishes the challenging large clamp and extra-large clamp and estimates their poses well. Our model is also robust in heavily occluded scenes. 
}
\vspace{-0.2cm}
\label{fig:compare_fig}
\end{figure*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\mnpsCa}{0.36}
\newcommand{\gwCa}{1.1}
\begin{figure}[htbp]
\centering

\subfigure[Ground Truth]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/gt_fmsk_41.png}\\
        % \vspace{0.02cm}
        %\caption{large clamp}
    \end{minipage}%
}%
\subfigure[PoseCNN]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/pcnn_msk_41.png}\\
        % \vspace{0.02cm}
        %\caption{large clamp}
    \end{minipage}%
}%
\subfigure[Mask R-CNN]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/msk_cnn_41.png}\\
        % \vspace{0.02cm}
        %\caption{large clamp}
    \end{minipage}%
}%

\subfigure[PVN3D($\mathcal{M_S}$)]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/onlyseg_msk_41.png}\\
        % \vspace{0.02cm}
        % \vspace{0.02cm}
        %\caption{extra-large clamp}
    \end{minipage}%
}%
\subfigure[PVN3D($\mathcal{M_{S,K}}$)]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/pv_msk_41.png}\\
        % \vspace{0.02cm}
        % \vspace{0.02cm}
        %\caption{extra-large clamp}
    \end{minipage}%
}%
\subfigure[PVN3D($\mathcal{M_{S,K,C}}$)]{
    \begin{minipage}[t]{\mnpsCa\linewidth}
        \centering
        \includegraphics[width=\gwCa in]{images/seg/cm_msk_41.png}\\
        % \vspace{0.02cm}
        % \vspace{0.02cm}
        %\caption{extra-large clamp}
    \end{minipage}%
}%
\centering
\caption{
    \textbf{Qualitative results of semantic segmentation on the YCB-Video dataset.} (b) shows the ground truth label. Different objects are labeled in different color, with large clamp colored green and extra-large clamp colored orange. In (c), the simple baseline Mask-RCNN is confused by the two objects. In (d), our semantic segmentation module $\mathcal{H}$, trained separately, can not distinguish them well either. In (e), jointly training $\mathcal{H}$ with the keypoints offset voting module $\mathcal{G}$ performs better. In (f), with the voted center and Mean-Shift clustering algorithm, our model can distinguish them well.
}
\vspace{-0.2cm}
\label{fig:tmp}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
    \renewcommand{\arraystretch}{1.5}
    \begin{table*}[tp]
        \centering
        \fontsize{8.5}{8}\selectfont
        \label{tab:YCB_PFM}
        \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
            \hline
            % \multirow{2}{*}{Object}&
             \  & \multicolumn{2}{c|}{PoseCNN+ICP\cite{xiang2017posecnn}} &\multicolumn{2}{c|}{PointFusion\cite{xu2018pointfusion}} &\multicolumn{2}{c|}{DCF\cite{}} &\multicolumn{2}{c|}{DF(per-pixel)\cite{wang2019densefusion}} &\multicolumn{2}{c}{Ours}\cr\cline{1-9}
             \  &ADD-S &ADD &ADD-S &ADD &ADD-S &ADD &ADD-S &ADD \cr
            \hline
            Object                         & ADDS        & ADD(S)        & ADDS          & ADD(S)          & ADDs      & ADD(S)      & ADDS           & ADD(S)           & ADDS          & ADD(S)        & ADDS          & ADD(S)        \cr\hline
            002 master chef can            & 83.9        & 50.2          & 90.9          & -               & 90.9      & 74.6        & 95.3           & 70.7             & 96.0          & 80.5          & \textbf{96.3} & \textbf{80.6} \\
            003 cracker box                & 76.9        & 53.1          & 80.5          & -               & 87.1      & 79.3        & 92.5           & 86.9             & 96.1          & \textbf{94.8} & \textbf{96.3} & 94.6          \\
            004 sugar box                  & 84.2        & 68.4          & 90.4          & -               & 94.3      & 84.2        & 95.1           & 90.8             & 97.4          & 96.3          & \textbf{97.6} & \textbf{96.6} \\
            005 tomato soup can            & 81.0        & 66.2          & 91.9          & -               & 90.5      & 79.8        & 93.8           & 84.7             & \textbf{96.2} & 88.5          & 95.6          & \textbf{89.6} \\
            006 mustard bottle             & 90.4        & 81.0          & 88.5          & -               & 90.6      & 83.5        & 95.8           & 90.9             & 97.5          & 96.2          & \textbf{97.8} & \textbf{97.0} \\
            007 tuna fish can              & 88.0        & 70.7          & 93.8          & -               & 91.7      & 73.8        & 95.7           & 79.6             & 96.0          & \textbf{89.3} & \textbf{96.8} & 88.9          \\
            008 pudding box                & 79.1        & 62.7          & 87.5          & -               & 89.3      & 84.1        & 94.3           & 89.3             & \textbf{97.1} & \textbf{95.7} & \textbf{97.1} & 94.6          \\
            009 gelatin box                & 87.2        & 75.2          & 95.0          & -               & 92.9      & 89.5        & 97.2           & 95.8             & 97.7          & 96.1          & \textbf{98.1} & \textbf{96.9} \\
            010 potted meat can            & 78.5        & 59.5          & 86.4          & -               & 83.2      & 74.6        & 89.3           & 79.6             & 93.3          & \textbf{88.6} & \textbf{94.7} & 88.1          \\
            011 banana                     & 86.0        & 72.3          & 84.7          & -               & 84.8      & 71.0        & 90.0           & 76.7             & 96.6          & 93.7          & \textbf{97.2} & \textbf{94.9} \\
            019 pitcher base               & 77.0        & 53.3          & 85.5          & -               & 89.5      & 80.3        & 93.6           & 87.1             & 97.4          & 96.5          & \textbf{97.6} & \textbf{96.9} \\
            021 bleach cleanser            & 71.6        & 50.3          & 81.0          & -               & 88.4      & 79.8        & 94.4           & 87.5             & 96.0          & 93.2          & \textbf{96.8} & \textbf{94.8} \\
            \textbf{024 bowl}              & 69.6        & 69.6          & 75.7          & 75.7            & 80.3      & 80.3        & 86.0           & 86.0             & 90.2          & 90.2          & \textbf{96.3} & \textbf{96.3} \\
            025 mug                        & 78.2        & 58.5          & 94.2          & -               & 90.7      & 76.6        & 95.3           & 83.8             & \textbf{97.6} & \textbf{95.4} & 97.3          & 94.2          \\
            035 power drill                & 72.7        & 55.3          & 71.5          & -               & 87.4      & 78.4        & 92.1           & 83.7             & 96.7          & 95.1          & \textbf{97.2} & \textbf{95.9} \\
            \textbf{036 wood block}        & 64.3        & 64.3          & 68.1          & 68.1            & 84.2      & 84.2        & 89.5           & 89.5             & 90.4          & 90.4          & \textbf{92.6} & \textbf{92.6} \\
            037 scissors                   & 56.9        & 35.8          & 76.7          & -               & 84.2      & 70.3        & 90.1           & 77.4             & 96.7          & 92.7          & \textbf{97.7} & \textbf{95.7} \\
            040 large marker               & 71.7        & 58.3          & 87.9          & -               & 89.5      & 81.0        & 95.1           & 89.1             & \textbf{96.7} & \textbf{91.8} & 96.6          & 89.1          \\
            \textbf{051 large clamp}       & 50.2        & 50.2          & 65.9          & 65.9            & 63.6      & 63.6        & 71.5           & 71.5             & 93.6          & 93.6          & \textbf{96.8} & \textbf{96.8} \\
            \textbf{052 extra large clamp} & 44.1        & 44.1          & 60.4          & 60.4            & 64.4      & 64.4        & 70.2           & 70.2             & 88.4          & 88.4          & \textbf{96.0} & \textbf{96.0} \\
            \textbf{061 foam brick}        & 88.0        & 88.0          & 91.8          & 91.8            & 83.1      & 83.1        & 92.2           & 92.2             & 96.8          & 96.8          & \textbf{97.3} & \textbf{97.3} \cr\hline
            ALL                            & 75.8        & 59.9          & 83.9          & -               & 85.7      & 77.9        & 91.2           & 82.9             & 95.5          & 91.8          & \textbf{96.6} & \textbf{92.7}
            \cr\hline
        \end{tabular}
        \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset. Objects with bold name are symmetric.}
    \end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% with ADD-S < 2cm
\begin{comment}
    \renewcommand{\arraystretch}{1.5}
    \begin{table*}[tp]
        \centering
        \fontsize{8.5}{8}\selectfont
        \label{tab:YCB_PFM}
        \begin{tabular}{l|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}|C{1.0cm}}
            \hline
            % \multirow{2}{*}{Object}&
             \  & \multicolumn{3}{c|}{PoseCNN + ICP}&\multicolumn{3}{c|}{DenseFusion (iterative)}&\multicolumn{3}{c}{PVN3D}\cr\cline{1-10}
             \  &ADDS &ADD &$<$2cm &ADDS &ADD &$<$2cm &ADDS &ADD &$<$2cm \cr
            \hline
            002\_master\_che\_can       &95.8 	&69.0 	&100.0 	&96.4 	&74.4 	&100.0 	&96.0 	&80.5 	&100.0 \cr%\hline
            003\_cracker\_box	        &92.7 	&80.7 	&91.6 	&95.5 	&93.9 	&99.5 	&96.1 	&94.8 	&100.0 \cr%\hline
            004\_sugar\_box	            &98.2 	&97.2 	&100.0 	&97.5 	&97.1 	&100.0 	&97.4 	&96.3 	&100.0 \cr%\hline
            005\_tomato\_soup\_can	    &94.5 	&81.6 	&96.9 	&94.6 	&88.2 	&96.9 	&95.6 	&88.6 	&98.1 \cr%\hline
            006\_mustard\_bottle	    &98.6 	&97.0 	&100.0 	&97.2 	&96.6 	&100.0 	&97.5 	&96.2 	&100.0 \cr%\hline
            007\_tuna\_fish\_can	    &97.1 	&83.1 	&100.0 	&96.6 	&82.1 	&100.0 	&95.8 	&89.0 	&100.0 \cr%\hline
            008\_pudding\_box	        &97.9 	&96.6 	&100.0 	&96.5 	&96.0 	&100.0 	&97.2 	&95.7 	&100.0 \cr%\hline
            009\_gelatin\_box	        &98.8 	&98.2 	&100.0 	&98.1 	&98.2 	&100.0 	&97.7 	&96.0 	&100.0 \cr%\hline
            010\_potted\_meat\_can	    &92.7 	&83.8 	&93.6 	&91.3 	&84.8 	&93.1 	&93.8 	&88.6 	&94.6 \cr%\hline
            011\_banana	                &97.1 	&91.6 	&99.7 	&96.6 	&78.2 	&100.0 	&96.7 	&94.0 	&100.0 \cr%\hline
            019\_pitcher\_base	        &97.8 	&96.7 	&100.0 	&97.1 	&97.3 	&100.0 	&97.4 	&96.5 	&100.0 \cr%\hline
            021\_bleach\_cleanser	    &96.9 	&92.3 	&99.4 	&95.8 	&94.9 	&100.0 	&96.0 	&93.2 	&100.0 \cr%\hline
            024\_bowl	                &81.0 	&17.5 	&54.9 	&88.2 	&5.6 	&98.8 	&90.6 	&38.6 	&85.7 \cr%\hline
            025\_mug	                &95.0 	&81.4 	&99.8 	&97.1 	&94.0 	&100.0 	&97.6 	&95.4 	&100.0 \cr%\hline
            035\_power\_drill	        &98.2 	&96.9 	&99.6 	&96.0 	&96.5 	&98.7 	&96.7 	&95.1 	&100.0 \cr%\hline
            036\_wood\_block	        &87.6 	&79.2 	&80.2 	&89.7 	&34.5 	&94.6 	&90.4 	&38.7 	&94.6 \cr%\hline
            037\_scissors	            &91.7 	&78.4 	&95.6 	&95.2 	&82.6 	&100.0 	&96.6 	&92.3 	&100.0 \cr%\hline
            040\_large\_marker	        &97.2 	&85.4 	&99.7 	&97.5 	&94.2 	&100.0 	&96.7 	&91.8 	&100.0 \cr%\hline
            051\_large\_clamp	        &75.2 	&52.6 	&74.9 	&90.3 	&31.4 	&98.0  	&93.6 	&71.6 	&98.9 \cr%\hline
            052\_extra\_large\_clamp	&64.4 	&28.7 	&48.8 	&74.9 	&30.7 	&86.4  	&85.7 	&62.7 	&90.6 \cr%\hline
            061\_foam\_brick	        &97.2 	&48.3 	&100.0 	&92.5 	&58.2 	&100.0 	&96.8 	&88.6 	&100.0 \cr\hline
            MEAN	                    &93.0 	&79.3 	&93.2 	&94.0 	&76.6 	&98.4  	&{\bf95.3} 	&{\bf85.0} 	&{\bf98.2} \cr
            \hline
        \end{tabular}
        \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset. Objects with bold name are symmetric.}
    \end{table*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%

\renewcommand{\arraystretch}{1.5}
\begin{table*}[tp]
    \centering
    \fontsize{8.5}{8}\selectfont
    \caption{Quantitative evaluation of 6D Pose on YCB-Video Dataset with diffrent formulation.}
    \label{tab:YCB_FM}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        % \multirow{2}{*}{Object}&
         \  & \multicolumn{2}{c|}{DF(RT)} & \multicolumn{2}{c|}{DF(3D KP)} 
         &\multicolumn{2}{c|}{Ours(RT)}&\multicolumn{2}{c|}{Ours(2D KP)}
         &\multicolumn{2}{c|}{Ours(Corr)}&\multicolumn{2}{c}{Ours(3D KP)}\cr\cline{1-13}
         \  &ADDS &ADD &ADDS &ADD &ADDS &ADD &ADDS &ADD &ADDS &ADD &ADDS &ADD\cr
        \hline
        002\_master\_che\_can     &95.8 	&69.0 	&100.0 	&96.4 	&74.4 	&100.0 	&96.0 	&80.5 	&100.0 \cr%\hline
        003\_cracker\_box	        &92.7 	&80.7 	&91.6 	&95.5 	&93.9 	&99.5 	&96.1 	&94.8 	&100.0 \cr%\hline
        004\_sugar\_box	        &98.2 	&97.2 	&100.0 	&97.5 	&97.1 	&100.0 	&97.4 	&96.3 	&100.0 \cr%\hline
        005\_tomato\_soup\_can	    &94.5 	&81.6 	&96.9 	&94.6 	&88.2 	&96.9 	&95.6 	&88.6 	&98.1 \cr%\hline
        006\_mustard\_bottle	    &98.6 	&97.0 	&100.0 	&97.2 	&96.6 	&100.0 	&97.5 	&96.2 	&100.0 \cr%\hline
        007\_tuna\_fish\_can	    &97.1 	&83.1 	&100.0 	&96.6 	&82.1 	&100.0 	&95.8 	&89.0 	&100.0 \cr%\hline
        008\_pudding\_box	        &97.9 	&96.6 	&100.0 	&96.5 	&96.0 	&100.0 	&97.2 	&95.7 	&100.0 \cr%\hline
        009\_gelatin\_box	        &98.8 	&98.2 	&100.0 	&98.1 	&98.2 	&100.0 	&97.7 	&96.0 	&100.0 \cr%\hline
        010\_potted\_meat\_can	    &92.7 	&83.8 	&93.6 	&91.3 	&84.8 	&93.1 	&93.8 	&88.6 	&94.6 \cr%\hline
        011\_banana	            &97.1 	&91.6 	&99.7 	&96.6 	&78.2 	&100.0 	&96.7 	&94.0 	&100.0 \cr%\hline
        019\_pitcher\_base	    &97.8 	&96.7 	&100.0 	&97.1 	&97.3 	&100.0 	&97.4 	&96.5 	&100.0 \cr%\hline
        021\_bleach\_cleanser	    &96.9 	&92.3 	&99.4 	&95.8 	&94.9 	&100.0 	&96.0 	&93.2 	&100.0 \cr%\hline
        024\_bowl	            &81.0 	&17.5 	&54.9 	&88.2 	&5.6 	&98.8 	&90.6 	&38.6 	&85.7 \cr%\hline
        025\_mug	                &95.0 	&81.4 	&99.8 	&97.1 	&94.0 	&100.0 	&97.6 	&95.4 	&100.0 \cr%\hline
        035\_power\_drill	        &98.2 	&96.9 	&99.6 	&96.0 	&96.5 	&98.7 	&96.7 	&95.1 	&100.0 \cr%\hline
        036\_wood\_block	        &87.6 	&79.2 	&80.2 	&89.7 	&34.5 	&94.6 	&90.4 	&38.7 	&94.6 \cr%\hline
        037\_scissors	        &91.7 	&78.4 	&95.6 	&95.2 	&82.6 	&100.0 	&96.6 	&92.3 	&100.0 \cr%\hline
        040\_large\_marker	    &97.2 	&85.4 	&99.7 	&97.5 	&94.2 	&100.0 	&96.7 	&91.8 	&100.0 \cr%\hline
        051\_large\_clamp	        &75.2 	&52.6 	&74.9 	&72.9 	&31.4 	&79.2 	&93.6 	&71.6 	&98.9 \cr%\hline
        052\_extra\_large\_clamp	&64.4 	&28.7 	&48.8 	&69.8 	&30.7 	&76.3 	&85.7 	&62.7 	&90.6 \cr%\hline
        061\_foam\_brick	        &97.2 	&48.3 	&100.0 	&92.5 	&58.2 	&100.0 	&96.8 	&88.6 	&100.0 \cr\hline
        MEAN	                &93.0 	&79.3 	&93.2 	&93.0 	&76.6 	&96.8 	&{\bf95.3} 	&{\bf85.0} 	&{\bf98.2} \cr
        \hline
    \end{tabular}
\end{table*}
%%%%

